Bridging the Communication Gap: Evaluating AI Labeling Practices for Trustworthy AI Development

As artificial intelligence (AI) becomes integral to economy and society, communication gaps between developers, users, and stakeholders hinder trust and informed decision-making. High-level AI labels, inspired by frameworks like EU energy labels, have been proposed to make the properties of AI models more transparent. Without requiring deep technical expertise, they can inform on the trade-off between predictive performance and resource efficiency. However, the practical benefits and limitations of AI labeling remain underexplored. This study evaluates AI labeling through qualitative interviews along four key research questions. Based on thematic analysis and inductive coding, we found a broad range of practitioners to be interested in AI labeling (RQ1). They see benefits for alleviating communication gaps and aiding non-expert decision-makers, however limitations, misunderstandings, and suggestions for improvement were also discussed (RQ2). Compared to other reporting formats, interviewees positively evaluated the reduced complexity of labels, increasing overall comprehensibility (RQ3). Trust was influenced most by usability and the credibility of the responsible labeling authority, with mixed preferences for self-certification versus third-party certification (RQ4). Our Insights highlight that AI labels pose a trade-off between simplicity and complexity, which could be resolved by developing customizable and interactive labeling frameworks to address diverse user needs. Transparent labeling of resource efficiency also nudged interviewee priorities towards paying more attention to sustainability aspects during AI development. This study validates AI labels as a valuable tool for enhancing trust and communication in AI, offering actionable guidelines for their refinement and standardization.

==> material/codes_Q1_AI_Use_Cases.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{AI Use Cases (0+41)} [.{Others (6)} ] [.{Digitalization \& Automation (5)} ] [.{Health \& Medicine (5)} ] [.{Organization \& Management (6)} ] [.{In-House Services (7)} ] [.{Manufacturing \& Industry (3+9)} [.{Production Monitoring (4)} ] [.{Predictive Maintenance (5)} ] ] ]
\end{tikzpicture}

==> material/codes_Q1_ML_Methods.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{ML Methods (1+63)} [.{Others (2)} ] [.{Unsupervised \& Clustering (3)} ] [.{Computer Vision (5)} ] [.{Natural Language Processing (9)} ] [.{Traditional AI (ML \& Training Models) (15)} ] [.{AI-as-a-Service (Pretrained \& GenAI) (29)} ] ]
\end{tikzpicture}

==> material/codes_Q1_ML_Tools_and_Brands.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{ML Tools \& Brands (1+35)} [.{Others (3)} ] [.{PyTorch (3)} ] [.{AWS (3)} ] [.{Azure (5)} ] [.{TensorFlow (5)} ] [.{ScikitLearn (7)} ] [.{OpenAI (9)} ] ]
\end{tikzpicture}

==> material/codes_Q1_Types_of_Daily_Work.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{Types of Daily Work (1+63)} [.{Others (2)} ] [.{Marketing \& Networking (3)} ] [.{UX Design (4)} ] [.{Business Understanding (6)} ] [.{ML Engineering (6)} ] [.{Data Exploration \& Analysis (8)} ] [.{Consulting (9)} ] [.{Operation \& Infrastructure (11)} ] [.{Software Development (14)} ] ]
\end{tikzpicture}

==> material/codes_Q2_Associations.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{Associations (1+30)} [.{Others (2)} ] [.{Association: Energy Labels (14)} ] [.{Association: Nutri Score (14)} ] ]
\end{tikzpicture}

==> material/codes_Q2_Property_Importance.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{Property Importance (1+63)} [.{Consistency \& Robustness (5)} ] [.{Up-to-dateness \& Usability (7)} ] [.{Temporal Performance (11)} ] [.{Predictive Quality (20)} ] [.{Energy, Resources \& Sustainability (20)} ] ]
\end{tikzpicture}

==> material/codes_Q2_Target_Audience.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{Target Audience (10)} ]
\end{tikzpicture}

==> material/codes_Q3_General_Comparison.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{General Comparison (0+46)} [.{Others (1)} ] [.{Compet Less Reliable or Relevant (Negative) (3)} ] [.{Compet More In-Depth (Positive) (13)} ] [.{Compet Rather Complex (Negative) (29)} ] ]
\end{tikzpicture}

==> material/codes_Q3_Workflows_and_Use.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{Workflows and Use (5+56)} [.{Others (5)} ] [.{Used: Code Repos (3)} ] [.{Requirements (4)} ] [.{Used: Model Cards (4)} ] [.{Used: Asking Experts (5)} ] [.{Used: Library Documentation (6)} ] [.{Used: Google (7)} ] [.{Used: Paper (8)} ] [.{Used: Blogs and Journalists (14)} ] ]
\end{tikzpicture}

==> material/codes_Q4_Dimensions_of_Trust.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{Dimensions of Trust (4+62)} [.{Others (9)} ] [.{Regulation Skepticism (4)} ] [.{Distrust in Labels (7)} ] [.{Trust and Privacy (7)} ] [.{Distrust in Authorities (8)} ] [.{Trust in Labels (11)} ] [.{General AI Skepticism (16)} ] ]
\end{tikzpicture}

==> material/codes_Q4_Who_Needs_Trust.tex <==
\begin{tikzpicture}[grow=right,level distance=180pt,scale=1,transform shape]
\Tree [.{Who Needs Trust (1+25)} [.{Developers of AI (6)} ] [.{End-Users of AI (8)} ] [.{Experts Using AI (11)} ] ]
\end{tikzpicture}
